Joining datasets via data augmentation in the label space for neural networks

Most, if not all, modern deep learning systems restrict themselves to a single dataset for neural network training and inference. In this article, we are interested in systematic ways to join datasets that are made of similar purposes. Unlike previous published works that ubiquitously conduct the dataset joining in the uninterpretable latent vectorial space, the core to our method is an augmentation procedure in the label space. The primary challenge to address the label space for dataset joining is the discrepancy between labels: non-overlapping label annotation sets, different labeling granularity or hierarchy and etc. Notably we propose a new technique leveraging artificially created knowledge graph, recurrent neural networks and policy gradient that successfully achieve the dataset joining in the label space. Empirical results on both image and text classification justify the validity of our approach.

==> app.tex <==
\section{Appendix}

\subsection{Architecture details}
As a further explanation of the model architecture, we plot the conceptual attention module in Figure~\ref{app:fig:arch}.

\begin{figure*}[h]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=1.5\columnwidth]{multi-head.png}}
\caption{Multi-head attention module architecture.}
\label{app:fig:arch}
\end{center}
\vskip -0.2in
\end{figure*}

\subsection{Experiments}
All experiments are implemented by Python 3.8 and Pytorch 1.5.1. 
We run each of the experiments on an NVIDIA GeForce RTX 2080Ti GPU.
Primarily we use the default Adam optimizer to train our model.
The other training details are revealed in Table~\ref{app:tab:ours}.

\subsection{Comparison experiments}
In Table~\ref{app:tab:ffn} and~\ref{app:tab:pseudo}, we reveal the settings for the baseline experiments.
For the ablation study in Section~\ref{subsec:ablation}, we use the same settings as in the previous section while altering the considered factors.

\begin{table*}[h]
\caption{Training settings for the classification experiments of our label space augmentation approach (\textit{\textbf{label-aug}}).  \textit{\textbf{LRE}} and \textit{\textbf{LR}} indicate the learning rate adopted for the encoder backbone (\textit{EfficientNet-B4} and \textit{BERT/LSTM} respectively for image and text experiments) and the rest of model parameters.
\textbf{\textit{Dymanic-Reduce(n)}} means we lower the learning rate by half when the dev set performance does not improve for a consecutive \textit{n} epochs.}
\vskip 0.15in
\begin{center}
\label{app:tab:ours}
\begin{small}
\begin{sc}
\begin{tabular}{lrrrrrrrrr}
\toprule
\textbf{Dataset}   & \textit{\textbf{Batch Size}} &  \textit{\textbf{Initial LRE}}  &\textit{\textbf{Initial LR}} & \textit{\textbf{Decay Period(epoch)}} & \textit{\textbf{Attention Size}} & \textit{\textbf{Hidden Size}} & \textit{\textbf{Input}} \\ 
\midrule
 \textit{Oxford-IIIT Pet}     & 8   & 0.00005  & 0.0004 &  10 & 1024 & 1024 & 380*380\\  
 \textit{PetFusion}      & 24   & 0.0001  & 0.0004 & 10 & 1024 & 1024 & 380*380\\ 
 \textit{102 Category Flower}     & 12   & 0.0001  & 0.0005 & \textit{Dynamic Reduce(5)} & 1024 & 1024 & 380*380\\
 \textit{FlowerFusion}   & 12   & 0.0002  & 0.0006 & \textit{Dynamic Reduce(5)} & 1024 & 1024 & 380*380\\
 \textit{ArxivOriginal} & 128 & 0.000015 & 0.000015 & \textit{Dynamic Reduce(5)} & 768 & 768 & $\leq$512 \\
 \textit{ArxivFusion} & 128 & 0.000015 & 0.000015 & \textit{Dynamic Reduce(5)} & 768 & 768 & $\leq$512 \\
 \textit{ArxivOriginal-LSTM} & 128 & 0.0007 & 0.0007 & \textit{Dynamic Reduce(5)} & 768 & 768 & $\leq$512 \\
 \bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

\begin{table*}[h]
\caption{Training settings for baseline experiments. Namely the \textit{EfficientNet-B4 + FFN} and \textit{BERT/LSTM + FFN} experiments for image and text domain respectively.}
\vskip 0.15in
\begin{center}
\label{app:tab:ffn}
\begin{small}
\begin{sc}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Dataset}   & \textit{\textbf{Epoch}} & \textit{\textbf{Batch Size}} & \textit{\textbf{Input}} & \textit{\textbf{Initial LR}} & \textit{\textbf{Decay Period(epoch)}} \\ \midrule
 \textit{Oxford-IIIT Pet}     & 60   & 16  & 380*380 & 0.00005 & 10\\  
%  \textit{PetFusion} \jake{WHAT}     & 60   & 16  & 380*380 & 0.00005  & 10\\ 
 \textit{102 Category Flower}     & 60   & 16  & 380*380 & 0.0001  & \textit{Dynamic Reduce(5)}\\
%  \textit{FlowerFusion}   & 60   & 16  & 380*380 & 0.0001 & \textit{Dynamic Reduce(5)}\\ 
 \textit{ArxivOriginal} & 40 & 128 & $\leq$ 512 & 0.000015 & \textit{Dynamic Reduce(5)} \\
 \textit{ArxivFusion} & 40 & 128 & $\leq$ 512 & 0.000015 & \textit{Dynamic Reduce(5)} \\
 \textit{ArxivOriginal-LSTM} & 80 & 128 & $\leq$ 512 & 0.0007 & \textit{Dynamic Reduce(5)} \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

\begin{table*}[h]
\caption{Training settings for \textit{Pseudo Label} method.}
\vskip 0.15in
\begin{center}
\label{app:tab:pseudo}
\begin{small}
\begin{sc}
\begin{tabular}{lrrrrr}
\toprule
\textbf{Dataset}   & \textit{\textbf{Epoch}} & \textit{\textbf{Batch Size}} & \textit{\textbf{Input}} & \textit{\textbf{Initial LR}} & \textit{\textbf{Decay Period(epoch)}}\\ \midrule
 \textit{Oxford-IIIT Pet}     & 60   & 16  & 380*380 & 0.0001  & 10\\  
 \textit{PetFusion}     & 60   & 16  & 380*380 & 0.0001  & 10\\  
 \textit{102 Category Flower}   & 60   & 16  & 380*380 & 0.0004  & \textit{Dynamic Reduce(5)}\\ 
 \textit{FlowerFusion}   & 60   & 16  & 380*380 & 0.0004  & \textit{Dynamic Reduce(5)}\\ 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}





\subsection{Dataset statistics extended}
As extended from Table~\ref{tab:dataset}, in this section we provide some further details about the datasets and their label graphs.
\begin{enumerate}
    \item \textbf{Pet datasets}. We construct 14 augmented nodes in addition to the 39 label nodes extracted from both datasets. The total edge number is 119.
    \item \textbf{Flower datasets}. We augment the label graph by 18 intermediate nodes with a total edge number 129.
    \item \textbf{Arxiv}. We adopt the original Arxiv label hierarchy graph structuring the website~\footnote{http://arxiv.org/}. 
\end{enumerate}
Due to the size issues of these graphs, we only visualize the moderate-size graph of the Pet datasets in Figure~\ref{app:fig:extendedg}.
We will release the other label graphs in the format of metafiles upon publication.

\begin{figure*}[h]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=1.8\columnwidth]{ExtendGraph.png}}
\caption{Complete label graph for \textit{Pet datasets}. The red and green color denote augmented nodes at different hierarchies, and white color indicates label nodes. The dotted lines indicate nondeterministic paths.}
\label{app:fig:extendedg}
\end{center}
\vskip -0.2in
\end{figure*}



% \textbf{Cat-Dog-Classification}
% Smaller label graph(trimmed graph) is shown in Fig~\ref{fig:smaller} and graph with best results is shown in Fig~\ref{fig:extendedg}.

% \textbf{Flower-Classification}
% Since there are too many nodes in the flower label graph to show the graph by pictures clearly, we show the statistical information of nodes and edges in Table~\ref{tab:stat}.

% \begin{table}[h]
% \caption{Statistical information of nodes and edges for label graphs. \textit{\textbf{D-Edges}} and \textit{\textbf{ND-Edges}} are short for deterministic edges and nondeterministic edges respectively.}
% \vskip 0.15in
% \begin{center}
% \label{tab:stat}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lrrrrrr}
% \toprule
% \textbf{Label}   & \textit{\textbf{Label Nodes}} & \textit{\textbf{Augmented Nodes}} & \textit{\textbf{Total Nodes}} & \textit{\textbf{D-Edges}} & \textit{\textbf{ND-Edges}} & \textit{\textbf{Total Edges}}\\ \midrule
%  %\textit{Pet-Smaller}     & 1   & 39  & 4 & 44 & 43 & 0 & 43\\
%  \textit{Pet}       & 39  & 14 & 54 & 111 & 8 & 119\\ 
%  \textit{Flower}    & 111  & 18 & 130 & 129 & 0 & 129\\ 
%  \textit{Arxiv}     & 149 & 21 & 171 & 170 & 0 & 170 \\ 
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{figure*}[h]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{OriginGraph.jpg}}
% \caption{Smaller graph for \emph{Cat-Dog-Classification}. White nodes and green nodes are label nodes, and red nodes are intermediate nodes. The lines represent deterministic paths.}
% \label{fig:smaller}
% \end{center}
% \vskip -0.2in
% \end{figure*}


% \subsection{Experiment}
% \subsubsection{Image Classification}
% All experiments were implemented in Python 3.8 on Pytorch 1.5.1. All experiments were conducted on an Intel(R) Core(TM) i9-9900X CPU 3.50GHz processors (10 physical cores and 20 CPU threads) with 128GB RAM accelerated by a NVIDIA GeForce RTX 2080 Ti GPU. And we use Adam with $\beta_1$ = 0.9 and $\beta_2$ = 0.999 as global setting. And details architecture of multi-head attention module is shown in Fig~\ref{fig:arch}.


% \textbf{Basic Setting}
% Image Classification experiments settings in section 4.2 of paper are listed in Table~\ref{tab:ffn}, Table ~\ref{tab:pseudo} and Table ~\ref{tab:ours}.





% \textbf{Ablation Study Setting}
% Ablation study experiments settings in section 4.5 of paper are listed in Table~\ref{tab:graph} and Table ~\ref{tab:loss}.

% \begin{table}[h]
% \caption{Experiments in section 4.5 part 1 of paper are based on following settings. And the experiments share the settings: \textit{Epoch} 60;  \textit{Input Image Resolution} 380*380; \textit{LR Decay Rate} 0.5; \textit{gradient clip} 50. Note that, smaller graph and graph with best results share the same settings in the same dataset.}
% \vskip 0.15in
% \begin{center}
% \label{tab:graph}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lrrrrrrrr}
% \toprule
% \textbf{Dataset}   & \textit{\textbf{Batch Size}} &  \textit{\textbf{Initial LRE}}  &\textit{\textbf{Initial LRD}} & \textit{\textbf{Decay Period(epoch)}}  & \textit{\textbf{Attention Size}} & \textit{\textbf{Hidden Size}}\\ \midrule
%  \textit{Oxford-IIIT Pet}     & 8   & 0.00005  & 0.0004 &  10 & 1024 & 1024\\  
%  \textit{PetFusion}      & 24   & 0.0001  & 0.0004 & 10 & 1024 & 1024\\ 
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{table*}[h]
% \caption{Experiments in section 4.5 part 2 of paper are based on following settings. And the experiments share the settings: \textit{Epoch} 60;  \textit{Input Image Resolution} 380*380; \textit{LR Decay Rate} 0.5; \textit{gradient clip} 50.}
% \vskip 0.15in
% \begin{center}
% \label{tab:loss}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lrrrrrrrr}
% \toprule
% \textbf{Dataset}   & \textit{\textbf{Batch Size}} &  \textit{\textbf{Initial LRE}}  &\textit{\textbf{Initial LRD}} & \textit{\textbf{Decay Period(epoch)}}  & \textit{\textbf{Attention Size}} & \textit{\textbf{Hidden Size}}\\ \midrule
%  \textit{Oxford-IIIT Pet}     & 8   & 0.00005  & 0.0004 &  10 & 1024 & 1024\\  
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}




% % \vskip 0.3in
% \subsubsection{Text Classification}

% \end{document}


% This document was modified from the file originally made available by
% Pat Langley and Andrea Danyluk for ICML-2K. This version was created
% by Iain Murray in 2018, and modified by Alexandre Bouchard in
% 2019 and 2021. Previous contributors include Dan Roy, Lise Getoor and Tobias
% Scheffer, which was slightly modified from the 2010 version by
% Thorsten Joachims & Johannes Fuernkranz, slightly modified from the
% 2009 version by Kiri Wagstaff and Sam Roweis's 2008 version, which is
% slightly modified from Prasad Tadepalli's 2007 version which is a
% lightly changed version of the previous year's version by Andrew
% Moore, which was in turn edited from those of Kristian Kersting and
% Codrina Lauth. Alex Smola contributed to the algorithmic style files.

